Machine learning Hadron Spectral Functions in Lattice QCD

Hadron spectral functions carry all the information of hadrons and are encoded in the Euclidean two-point correlation functions. The extraction of hadron spectral functions from the correlator is a typical ill-posed inverse problem and infinite number of solutions to this problem exists. We propose a novel neural network (sVAE) based on the Variation Auto-Encoder (VAE) and Bayesian theorem. Inspired by the maximum entropy method (MEM) we construct the loss function of the neural work such that it includes a Shannon-Jaynes entropy term and a likelihood term. The sVAE is then trained to provide the most probable spectral functions. For the training samples of spectral function we used general spectral functions produced from the Gaussian Mixture Model. After the training is done we performed the mock data tests with input spectral functions consisting 1) only a free continuum, 2) only a resonance peak, 3) a resonance peak plus a free continuum and 4) a NRQCD motivated spectral function. From the mock data test we find that the sVAE in most cases is comparable to the maximum entropy method in the quality of reconstructing spectral functions and even outperforms the MEM in the case where the spectral function has sharp peaks with insufficient number of data points in the correlator. By applying to temporal correlation functions of charmonium in the pseudoscalar channel obtained in the quenched lattice QCD at 0.75 $T_c$ on $128^3\times96$ lattices and $1.5$ $T_c$ on $128^3\times48$ lattices, we find that the resonance peak of $\eta_c$ extracted from both the sVAE and MEM has a substantial dependence on the number of points in the temporal direction ($N_\tau$) adopted in the lattice simulation and $N_\tau$ larger than 48 is needed to resolve the fate of $\eta_c$ at 1.5 $T_c$.

==> Flow1.tikz.tex <==
\usetikzlibrary{arrows.meta}
\usetikzlibrary{positioning,calc}
\tikzset{%
%  >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
      base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=4cm, minimum height=1cm,
                           text centered, font=\sffamily},
       activityStarts/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=green!30},
       activityStarts1/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=red!30},
       KL/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=1.5cm,
                           text centered, font=\sffamily,fill=green!30},
    activityRuns/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=green!30},
         process/.style = {base, minimum width=2.5cm, fill=blue!15,
                           font=\ttfamily},
      functions/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=1cm,
                           text centered, font=\sffamily, fill=yellow!30},
}
\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
\resizebox{1\textwidth}{!}{% 
\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]
  % Specification of nodes (position, etc.)
  \coordinate (input);
  \node (PG)             [activityStarts]              {$G_{gt}$\\ $\rho_{gt}$};
  \node (Encoder1)     [process, right= 5mm of PG]          {Encoder 1};
%  \node (es1)      [activityStarts1,  right= 5mm of Encoder1]   {$\mu$, $\sigma$,\\$\pi$};
  \node (es1)      [activityStarts1,  right= 5mm of Encoder1]   {$Q(z|G_{gt},\rho_{gt})$};
   \node (Ghat)     [activityStarts, below of=PG]   {${G}$};
    \node (Encoder2)     [process, right of=Ghat]          {Encoder 2};
    \node (es2)      [activityStarts1, right= 5mm of Encoder2]   {$P(z|{G})$};
 %  \node (onResumeBlock)     [activityStarts, right of =es1]   {z\\z\\z\\z\\z};
%   \node (onResumeBlock)  [KL, right= 2 cm of {$(es1)!0.5!(es2)$}]   {\huge{$z$}\\(K-L divergence)}; 
   %\node (onResumeBlock)  [activityRuns, minimum height=1cm, right= 2 cm of {$(es1)!0.5!(es2)$}]  {sampling \large{$z$}}; 
   \node (onResumeBlock)  [activityRuns, minimum height=1cm, right= 5 mm of es1]  {sampling \large{$z$}}; 
      \node (Decoder)     [process, right= 5mm of onResumeBlock]   {Decoder};
        \node (alphaG)     [activityStarts, right= 5mm of Decoder]   {$\rho(z)\to G[\rho(z)]$\\$\alpha(z)$};
       %\node [activityStarts] at ($(Decoder.north east)!.5!(alphaG.north west)$) (rhoz) {$\rho(z)$}      
      % \node (es3)      [activityStarts1, right of=Decoder]   {$\mu$\\ $\sigma$};
      \node (KL)  [functions,   right=3.5 cm of es2]   {$KL$ divergence};
      \node (E)     [functions, right=5mm of alphaG]   {$E_{Q}[\log P(\rho|z, {G})]$};
       \node (lossfun)     [ functions, below of= E]   {Loss function};
      % \node (rhoz)     [activityStarts, above left = 2mm of E]   {$\rho(z)$};
   % Specification of lines between nodes specified above
  % with aditional nodes for description 
    \draw[->]             (PG) -- (Encoder1);
    \draw[->]             (Encoder1) -- (es1);
%    \draw[->]             (es1) -- node[xshift=-0.6cm, yshift=-0.65cm,text width=0.2cm]{sampling}(onResumeBlock);
    \draw[->]             (es1) -- (onResumeBlock);
    \draw[->]             (onResumeBlock) -- (Decoder);
      \draw[->]             (Ghat) -- (Encoder2);
      \draw[->]             (Encoder2) -- (es2);
       \draw[->]             (es2) -- (KL);
       \draw[->]             (alphaG) -- (E);      
       \draw[->]              (Decoder) -- (alphaG);
         \draw[->]             (E) -- (lossfun);
         \draw[->]             (KL) -- (lossfun); 
          \draw[->]             ([yshift=-5mm] es1.east) -- (KL);
  \end{tikzpicture}
  }
  
  

==> Flow2.tikz.tex <==
%\usetikzlibrary{arrows.meta}
%\usetikzlibrary{positioning,calc}

\tikzset{%
%  >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
      base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=4cm, minimum height=1cm,
                           text centered, font=\sffamily},
       activityStarts/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=1cm,
                           text centered, font=\sffamily, fill=green!30},
       activityStarts1/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=red!30},
       KL/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=1.5cm,
                           text centered, font=\sffamily,fill=green!30},
    activityRuns/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=green!30},
         process/.style = {base, minimum width=2.5cm, fill=blue!15,
                           font=\ttfamily},
}
\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
%\resizebox{0.35\textwidth}{!}{% 
\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]
  % Specification of nodes (position, etc.)
  \coordinate (input);
   \node (Ghat)     [activityRuns, below of=PG]   {${G}$};
    \node (Encoder2)     [process, right of=Ghat]          {Encoder 2};
    \node (es2)      [activityStarts1, right=6mm, at=(Encoder2.east)]   {$P(z|{G})$};
 %  \node (onResumeBlock)     [activityStarts, right of =es1]   {z\\z\\z\\z\\z};
 %  \node (onResumeBlock)  [activityRuns, right of = es2]   {$z$}; 
   \node (onResumeBlock)  [activityRuns, minimum height=1cm, right=6mm, at=(es2.east)]   {sampling \large{$z$}}; 
      \node (Decoder) [process, right=6mm,at=(onResumeBlock.east)]   {Decoder};
     %  \node (es3)      [activityStarts1, right of=Deconder]   {$\mu$\\ $\sigma$};
      \node (rho)     [activityRuns, minimum height=1cm, right=6mm, at=(Decoder.east)]   { $\rho(z)$\\$\alpha(z)$};
  % Specification of lines between nodes specified above
  % with aditional nodes for description 
    \draw[->]             (onResumeBlock) -- (Decoder);
      \draw[->]             (Ghat) -- (Encoder2);
      \draw[->]             (Encoder2) -- (es2);
%       \draw[->]             (es2) --  node[xshift=-0.5cm, yshift=0.3cm,text width=0.2cm]{sampling}(onResumeBlock);
       \draw[->]             (es2) --  node[xshift=0cm, yshift=0.3cm,text width=0cm]{}(onResumeBlock);
        \draw[->]             (Decoder) -- (rho);
       % \draw[->]             (es3) -- node[xshift=-0.5cm, yshift=0.3cm,text width=0.2cm]{sampling}(rho);
     %  \draw[->]            (es3)--(rho);
  \end{tikzpicture}
 % }
 
  
